Absolutely continuous spectrum for the Anderson model on a product of a tree with a finite graph

We prove the almost sure existence of absolutely continuous spectrum at low disorder for the Anderson model on the simplest example of a product of a regular tree with a finite graph. This graph contains loops of unbounded size.

==> intro.tex <==
\beginsection
\hd{Abstract}

We prove the almost sure existence of absolutely continuous spectrum at low disorder for the Anderson model on the simplest example of a product of a regular tree with a finite graph. This graph contains loops of unbounded size.

\hd{Introduction}

Since Klein's theorem on the existence of absolutely continuous spectrum for the Anderson model on a regular tree [K] was given new proofs, in [ASW] and [FHS], there have been several generalizations of this result to the Anderson model on other trees. For example, decorated trees was considered in [H] while substitution trees were treated in [KLW]. In this paper we show the almost sure existence of purely absolutely continuous spectrum at weak disorder for the Anderson model on the simplest example of a product of a regular tree with a finite graph. To our knowledge this is the first proof of extended states for the Anderson model on a graph with loops of unbounded size. Graphs with unbounded loops were considered in [FHS2] for other types of randomness.

The Laplace operator on the product of a regular tree with a finite graph is unitarily equivalent to a direct sum of shifted Laplace operators on the base tree, where the shifts are determined by the spectrum of the Laplacian on the finite factor graph. This implies that the spectrum of the Laplace operator is the union of shifted copies of the spectrum of the base tree Laplacian. What happens when a random potential of Anderson type is added?
In our example, we are able to prove the existence of absolutely continuous spectrum on 
the intersection of the shifted copies, namely,
the interval $[-2\sqrt{2}+1, 2\sqrt{2}-1]$. 
We conjecture that the analogous theorem is true for general products of trees with finite graphs. Notice, however, that if the norm of the finite factor graph Laplacian is too large, this intersection will be empty. It is an interesting open problem to determine the nature of the spectrum for energies where only some of the shifted copies of the Laplace operator in the decomposition of the free Laplacian have spectrum. In our example these would be the energies contained in the intervals $[-2\sqrt{2}, -2\sqrt{2}+1]$ and
$[2\sqrt{2}-1,2\sqrt{2}]$. The analogous problem for slowly decaying random potentials on the strip was considered in [FHS3], but the methods used there do not apply to the Anderson model. 

In this paper the base tree $T$ is a binary rooted tree and the finite factor graph $G$ is the graph with two vertices connected with a single edge. This graph $T\times G$ is depicted in Figure 1.

\vskip 20pt
\epsfxsize=5cm
\centerline{\epsffile{producttree1.eps}}
\centerline{\sl Figure 1}

The Laplacian for the product graph is $\L = \L_T\otimes 1 + 1\otimes\L_G$, acting on the Hilbert space $\ell^2(T\times G) = \ell^2(T)\otimes\ell^2(G) = \ell^2(T)\otimes\CC^2$. 
In what follows we will think of elements of $\ell^2(T)\otimes\CC^2$ as $\CC^2$ valued functions on $T$. From this point of view, the analysis of this model can be considered to be a $2\times 2$ matrix valued version of the model on the original tree. Roughly speaking, the hyperbolic plane $\HH$ is replaced by the Siegel upper half space $\SH_2$. So, although the outline of the proof is the same as for the tree, we are confronted with non-commuting variables and the much more complicated geometry at infinity of $\SH_2$.

For convenience we will actually work with the adjacency matrix, which amounts to setting the diagonal matrix elements of the Laplacian to zero. Then $\L_G = \twovec{0&1}{1&0}$, and the Laplacian acts on $\varphi\in \ell^2(T)\otimes\CC^2$ as
$$
\L\varphi(x) = \sum_{y:y\sim x} \varphi(y) + \L_G\varphi(x).
$$
Here $y\sim x$ means that $y$ is connected to $x$ by a single edge.

Let $Q$ denote an i.i.d.\ random potential on $T$ taking values in the set of $2\times 2$ real symmetric matrices ${\rm Sym}(2,\RR)$. Assume that the single site distribution is given by the measure $\nu$ satisfying

\be{Qhyp}
\EE\left[\|Q\|^{2(1+p)}\right] = \int_{{\rm Sym}(2,\RR)} \|Q\|^{2(1+p)} d\nu(Q) < \infty
\ee
for some $p>0$.

We study the spectral properties of the Anderson Hamiltonian
\be{AHam}
H_k = \L + k Q
\ee
for small coupling constant $k$, which we take to be positive. The goal of this paper is to prove the following theorem.

\begintheoremlabel{main} Let $H_k$ be the random Anderson Hamiltonian defined by \rf{AHam}, where the potential $Q$ satisfies \rf{Qhyp}. Let $I$ be any closed subinterval of $(-2\sqrt{2}+1,2\sqrt{2}-1)$. Then, for sufficiently small $k$, $H$ has purely absolutely continuous spectrum in $I$ almost surely. 
\endtheoremlabel

Here are some of the new ingredients in this paper. After a preliminary symplectic change of variables to move the fixed point of our recursion relation to $iI$, we define a weight function in \rf{weight2defn} with some extra convexity compared to the functions we used previously (the analogue on the original tree is described in the conference proceedings review [FHS4]). This allows a simple geometric characterization (\rf{rangecond} and \rf{eqcond}) of the places where our key inequality degenerates. This characterization involves an unusual co-ordinate system for $\SH_2$ given by \rf{Udefn}.


\hd{The forward Green function and the recursion relation}

Let $P$ denote the rank two projection onto the space of functions supported on the vertices above the root (inside the oval in Figure 1). Then, for $\lambda$ in the resolvent set of $H_k$, we define the Green function at the root to be
\be{gf}
G(\lambda) = P(H-\lambda)^{-1}P.
\ee


This Green function is a $\lambda$ dependent random variable taking values in the Siegel upper half space $\SH_2$.

By definition, $\SH_2$ is the set of symmetric $2\times 2$ matrices with complex entries whose imaginary parts are positive definite. The symplectic group ${\rm Sp}(4,\RR)$ acts on $\SH_2$ via generalized linear fractional transformations. For $\Gamma=\left[\matrix{A&B\cr C&D}\right]\in {\rm Sp}(4,\RR)$ and $Z\in \SH_2$ we write the action as $\Gamma\cdot Z = (AZ+B)(CZ+D)^{-1}$. Properties of $\SH_2$, its compactification, and the ${\rm Sp}(4,\RR)$ action that we need can be found in the thesis of Freitas [F].

The forward Green functions are defined by disconnecting the tree as indicated, and restricting the resolvent for the Hamiltonians of the two disconnected subtrees to the range of the projections corresponding to the root nodes of the subtrees. 

\vskip 20pt
\epsfxsize=5cm
\centerline{\epsffile{producttree2.eps}}
\centerline{\sl Figure 2}

\noindent The analogue of \rf{gf} gives rise to two forward Green functions $G_1(\lambda)$ and $G_2(\lambda)$ that, for a given realization of the potential
are related to $G(\lambda)$ by

\be{recursion}
G(\lambda) = \Phi_\lambda\left({{G_1(\lambda)+G_2(\lambda)}\over{2}}- {{k}\over{2}}Q\right)
\ee
where
$$
\Phi_\lambda(G) = (2G + \lambda - \L_G )^{-1}
$$
and $Q$ is the value of the potential at the root. Note that $\Phi_\lambda$ is the generalized linear fractional transformation which we can identify with the matrix
$$
\Phi_\lambda=\twovec{0& I/\sqrt{2}}{\sqrt{2}I&(\lambda I - \L_G)/\sqrt{2}}.
$$
If $\lambda$ is real, then $\Phi_\lambda\in {\rm Sp}(4,\RR)$. Otherwise, $\Phi_\lambda$ is a composition of a complex shift with a transformation in ${\rm Sp}(4,\RR)$.

We define $G_\lambda$ to be the fixed point of $\Phi_\lambda$. Solving the fixed point equation $G_\lambda = \Phi_\lambda(G_\lambda)$ yields
$$G_\lambda = -\left({{\lambda - \L_G}\over{4}}\right) + i \sqrt{{{1}\over{2}} - \left({{\lambda-\L_G}\over{4}}\right)^2}.$$
Since the eigenvalues of $\L_G$ are $\pm 1$, both eigenvalues of $G_\lambda$ lie on a circle of radius $1/\sqrt{2}$ in the upper half plane when $\lambda\in (-2\sqrt{2}+1, 2\sqrt{2}-1)$. For these values of $\lambda$, $G_\lambda \in \SH_2$, while for real $\lambda$ outside this range, $G_\lambda$ lies on the boundary at infinity. This explains the range of $\lambda$ for which we can prove absolutely continuous spectrum.

We now choose a closed interval $J \subset (-2\sqrt{2}+1, 2\sqrt{2}-1)$ that will remain fixed for the rest of the paper. Define 
\be{Rdefn}
R_\epsilon = \{\lambda\in\CC : \Re \lambda \in J, 0<\Im \lambda \le \epsilon\}
\ee
with $\epsilon$ sufficiently small so that $G_\lambda\in\SH_2$ for $\lambda\in R_\epsilon$.


We want the fixed point $G_\lambda$ to serve as an origin for $\SH_2$. To avoid difficulties that result from the fact that $G_\lambda$ does not commute with all of $\SH_2$, we perform a $\lambda$ dependent symplectic change of variables to move the origin to $iI$. For $\lambda\in R_\epsilon$, write $G_\lambda = X_\lambda + i Y_\lambda$ and let $\Gamma_\lambda$ be the symplectic transformation given by the matrix
$$
\Gamma_\lambda = \left[\matrix{Y_\lambda^{-1/2} & -Y_\lambda^{-1/2}X_\lambda\cr
0&Y_\lambda^{1/2}\cr}\right].
$$
Then $\Gamma_\lambda\cdot G_\lambda = iI$.
We will work with the new variables $Z$ in $\SH_2$ related to $G$ by
$$
Z = \Gamma_\lambda\cdot G = Y_\lambda^{-1/2}GY_\lambda^{-1/2}-Y_\lambda^{-1/2}X_\lambda Y_\lambda^{-1/2}.
$$
With these variables, equation \rf{recursion} becomes
\be{newrecursion}
Z(\lambda) = \Psi_\lambda\left({{Z_1(\lambda)+Z_2(\lambda)}\over{2}}- {{k}\over{2}}\widehat Q\right)
\ee
where $\Psi_\lambda = \Gamma_\lambda \circ \Phi_\lambda \circ \Gamma_\lambda^{-1}$ and $\widehat Q =  Y_\lambda^{-1/2}QY_\lambda^{-1/2}$. For future reference we compute the matrix for $\Psi_\lambda$ explicitly. This yields
\be{Psiformula}
\Psi_\lambda = \twovec{(\lambda-\L_G)/(2\sqrt{2}) & -\sqrt{1-(\lambda-\L_G)^2/8}}{\sqrt{1-(\lambda-\L_G)^2/8}&(\lambda-\L_G)/(2\sqrt{2})}
=\twovec{\cos(\Theta_\lambda) & -\sin(\Theta_\lambda)}{\sin(\Theta_\lambda) & \cos(\Theta_\lambda)}
\ee
where $\Theta_\lambda = \cos^{-1}((\lambda-\L_G)/(2\sqrt{2}))$ with the branch of $\cos^{-1}$ chosen to make $\sin(\Theta_\lambda)$ positive definite when $\lambda\in J$. Notice that $\Psi_\lambda$ is an orthogonal symplectic matrix for $\lambda \in J$.

Equation \rf{newrecursion}, and the self-similarity of the tree imply that for any positive measurable function $w$ on $\SH_2$, 
\be{probrecursion}
\Bbb E [ w(Z(\lambda)) ] = \Bbb E \left[ w\left(\Psi_\lambda\left({{Z_1(\lambda)+Z_2(\lambda)}\over{2}} - {{k}\over{2}}\widehat Q\right)\right) \right],
\ee
where $Z_1(\lambda)$, $Z_2(\lambda)$ are independent copies of $Z(\lambda)$ and $Q$ is independently distributed according to $\nu$.

\hd{The functions $w_p(Z_1,Z_2)$ and $\mu_{2,p}^*(Z_1,Z_2)$}

The following symplectically invariant function will play an important role in our analysis.
For $Z_j = X_j + i Y_j$, $j=1,2$  and $p>0$, let
\be{weight2defn}
w_{p}(Z_1,Z_2) = \|Y_2^{-1/2}(Z_1-Z_2)^*Y_1^{-1}(Z_1-Z_2)Y_2^{-1/2}\|_{1+p}^{1+p}
\ee
where $\|\cdot\|_{1+p}$ denotes the Schatten $(1+p)$ norm. When $p=0$ the norm gives the trace, and the resulting definition is a function of the Riemannian distance in the Siegel space. 
As we will see below, $w_p$ is still invariant under the symplectic action when $p>0$, and
the extra convexity that results for positive $p$ will be important. 

The weight function that we use to measure growth in $\SH_2$ is defined to be
\be{weightdefn}
w_{p}(Z) = w_{p}(Z,iI).
\ee

The following lemma collects some properties of $w_p(Z_1,Z_2)$ and $w_{p}(Z)$.

\beginlemmalabel{imwt} 

(i) Let $\Gamma$ be an element of $Sp(4,\RR)$ acting on $\SH_2$. Then
$$
w_p(\Gamma\cdot Z_1, \Gamma\cdot Z_2) = w_p(Z_1, Z_2).
$$

(ii) Let $T$ be a complex translation given by the action $T\cdot Z = Z+it$ with $t>0$. Then
$$
w_p(T\cdot Z_1,T\cdot Z_2) < w_p(Z_1, Z_2).
$$

(iii) There are constants $C_1$ and $C_2$ such that for every $Z\in \SH_2$, 
$$
\|\Im(Z)\|^{1+p} \le C_1 w_{p}(Z) + C_2.
$$

(iv) For any $\epsilon>0$ there exists $C_\epsilon$ such that for any $Q\in {\rm Sym}(2,\RR)$
$$
w_p(Z+Q) \le (1+\epsilon+C_\epsilon\|Q\|^{2(1+p)})w_p(Z) + C_\epsilon\|Q\|^{2(1+p)}.
$$
\endlemmalabel
\noindent This lemma is proved in Appendix 1.

The ratio
$$
\mu_{2,p,\lambda}(Z_1,Z_2) = {{w_p\left(\Psi_\lambda\left({{Z_1+Z_2}\over{2}}\right)\right)}\Big/{\left(\half w_p(Z_1)+\half w_p(Z_2)\right)}}
$$
plays a central role in our analysis. To understand this function we introduce an unusual co-ordinate system for $\SH_2$. For $Z=X+iY\in\SH_2$, define
\be{Udefn}
U(Z)=Y^{-1/2}(Z-iI).
\ee
We will study this co-ordinate system in detail below. Clearly $w_p(Z) = \|U(Z)^*U(Z)\|_{1+p}^{1+p}=\|U(Z)\|_{2(1+p)}^{2(1+p)}$. The quantity $U(Z)$ appears in the  following crucial formula.

\beginpropositionlabel{mainformula} For $\Im\lambda\ge 0$,
\be{mf}
w_p\left(\Psi_\lambda\left({{Z_1+Z_2}\over{2}}\right)\right) \le
\left\|\half 
\left[U(Z_1)^*,U(Z_2)^*\right]
P(Y_1,Y_2)
\left[\matrix{U(Z_1)\cr U(Z_2)}\right]
\right\|_{1+p}^{1+p}
\ee
where
$$
P(Y_1,Y_2) = \left[\matrix{Y_1^{1/2}\cr Y_2^{1/2}}\right]
(Y_1+Y_2)^{-1}
\left[Y_1^{1/2}, Y_2^{1/2}\right]
$$
is the orthogonal projection onto the range of $\left[\matrix{Y_1^{1/2}\cr Y_2^{1/2}}\right]$. The inequality is an equality if $\lambda\in\RR$.
\endpropositionlabel

Notice that the left side of \rf{mf} does not depend on $\lambda$, so we can define the $\lambda$ independent upper bound for $\mu_{2,p,\lambda}$.
$$
\mu_{2,p}^*(Z_1,Z_2) = \left\|\half 
\left[U(Z_1)^*,U(Z_2)^*\right]
P(Y_1,Y_2)
\left[\matrix{U(Z_1)\cr U(Z_2)}\right]
\right\|_{1+p}^{1+p}
\Big/{\left(\half w_p(Z_1)+\half w_p(Z_2)\right)}
$$
It follows from  \thmrf{mainformula} that 
\be{mucomp}
\mu_{2,p,\lambda}\le \mu_{2,p}^*.
\ee

\beginpropositionlabel{mainineq}
The ratio $\mu_{2,p}^*(Z_1,Z_2)\le 1$, or equivalently
\be{mainineq}
\left\|\half 
\left[U(Z_1)^*,U(Z_2)^*\right]
P(Y_1,Y_2)
\left[\matrix{U(Z_1)\cr U(Z_2)}\right]
\right\|_{1+p}^{1+p}
\le
\half w_p(Z_1)+\half w_p(Z_2).
\ee
Equality holds if and only if $Z_1=Z_2$.

\endpropositionlabel

These propositions are proved below, where we also determine in what form they survive on the compactifications considered below.

\hd{Reduction to estimates on $\mu_{2,p}^*$}

If $Z = \Gamma_\lambda\cdot G$ then $\Im G = \Yh_\lambda \Im Z\,\Yh_\lambda$. Thus, $\|\Im G\| \le C\|\Im Z\|$ uniformly for $\lambda \in R_\epsilon$ with $\epsilon$ small. So, given \thmrf{imwt} (iii), \thmrf{main} follows from the following theorem (see, e.g., Lemma 1 of [FHS2]).

\begintheoremlabel{mainest}
Let $G(\lambda)$ be the Green function for the random Hamiltonian $H_k=\L + k Q$ defined by \rf{gf}, and let $Z(\lambda)=\Gamma_\lambda\cdot G(\lambda)$. Then, for sufficiently small coupling constant $k$, and small $\epsilon$,  there exists a constant $C$ such that
$$
\sup_{\lambda\in R_\epsilon} \Bbb E [ w_{p}(Z(\lambda)) ] \le C.
$$
\endtheoremlabel

In this section we will indicate how this theorem follows from estimates of $\mu_{2,p}^*$ at infinity. This part of the proof follows the same lines as [FHS]. Using \rf{probrecursion} twice 
we find that
$$
\EE[w_p(Z(\lambda))]=
\EE\left[w_p\left(
\Psi_\lambda\left(
\half Z_{1} + 
\half\Psi_\lambda\left(\half Z_{2}+\half Z_{3} - \half k\widehat Q_2
\right) - \half k\widehat Q_1
\right)
\right)
\right]
$$
where $Z_1$, $Z_2$  and $Z_3$ are independent copies of $Z(\lambda)$ and $Q_1$ and $Q_2$ are independent copies of the single site (matrix) potential. Since we may permute $Z_1$, $Z_2$  and $Z_3$ without changing the expectation, we find
$$
\EE[w_p(Z(\lambda))] = {{1}\over{3}} \EE\left[\Sigma\Big(Z_1,Z_2,Z_3,k\widehat Q_1,k\widehat Q_2,\lambda\Big)\right]
$$
where $\Sigma$ is the symmetrization of the expression above given by
$$
\Sigma\Big(Z_1,Z_2,Z_3,Q_1,Q_2,\lambda\Big) =
\sum_{\sigma}
w_p\left(
\Psi_\lambda\left(
\half Z_{\sigma_1} + 
\half\Psi_\lambda\left(\half Z_{\sigma_2}+\half Z_{\sigma_3} - \half Q_2
\right) - \half Q_1
\right)
\right).
$$
In the sum, $\sigma$ ranges over the three cyclic permutations of $(1,2,3)$.

Introduce the ratio
$$
\mu_3\Big(Z_1,Z_2,Z_3,Q_1,Q_2,\lambda\Big)
={{\Sigma\Big(Z_1,Z_2,Z_3,Q_1,Q_2,\lambda\Big)}
\over
{w_p(Z_1) + w_p(Z_2) + w_p(Z_3)}}.
$$
To prove our main theorem, we will prove that
\beginpropositionlabel{mu3est} There exists a compact set $K\subseteq \SH_2\times\SH_2\times\SH_2$, $\epsilon>0$, 
$\epsilon_1>0$ and $\delta >0$ so that
$$
\sup_{(Z_1,Z_2,Z_3)\not\in K,\|Q_1\|\le \epsilon_1,\|Q_2\|\le \epsilon_1,\lambda\in R_\epsilon}
\mu_3\Big(Z_1,Z_2,Z_3,Q_1,Q_2,\lambda\Big) \le (1-\delta).
$$
\endpropositionlabel
Given \thmrf{mu3est} we can prove \thmrf{mainest} as follows.
\beginproofof{\thmrf{mainest}}
Choose $\epsilon$, $\epsilon_1$, $K$ and $\delta$ so that the estimate in \thmrf{mu3est} holds.
Let $\chi(\cdot)$ denote the characteristic function of the indicated set. We can then estimate
$\EE[w_p(Z(\lambda))]$ by introducting cutoffs as follows.
\be{cutoffest}\eqalign{
\EE[w_p(Z(\lambda))]
&\le {{1}\over{3}}\EE\left[\chi\Big(\|k\widehat Q_1\| \le \epsilon_1,\|k\widehat Q_2\| \le \epsilon_1, (Z_1,Z_2,Z_3)\not\in K\Big)\Sigma\right]\cr
&\quad +{{1}\over{3}}\EE\left[\chi\Big(\|k\widehat Q_1\| \le \epsilon_1,\|k\widehat Q_2\| \le \epsilon_1, (Z_1,Z_2,Z_3)\in K\Big)\Sigma \right]\cr
&\quad +{{1}\over{3}}\EE\left[\chi\Big(\|k\widehat Q_1\| > \epsilon_1\Big)\Sigma \right]\cr
&\quad +{{1}\over{3}}\EE\left[\chi\Big(\|k\widehat Q_2\| > \epsilon_1\Big)\Sigma \right]\cr
}\ee
Here $\Sigma$ stands for $\Sigma\Big(Z_1,Z_2,Z_3,k\widehat Q_1,k\widehat Q_2,\lambda\Big)$.
In the first term on the right of \rf{cutoffest} we may replace $\Sigma$ with
$(1-\delta)(w_p(Z_1) + w_p(Z_2) + w_p(Z_3))$ for any $\lambda\in R_\epsilon$, thanks to $\thmrf{mu3est}$. This results in the following estimate for the first term on the right of \rf{cutoffest}, valid for all $\lambda\in R_\epsilon$.
$$
{{1}\over{3}}\EE\left[\chi\Big(\|k\widehat Q_1\| \le \epsilon_1,\|k\widehat Q_2\| \le \epsilon_1, (Z_1,Z_2,Z_3)\not\in K\Big)\Sigma\right]
\le (1-\delta)\EE[w_p(Z(\lambda))].
$$

The second term in the right of \rf{cutoffest} is estimated by noting that $\Sigma\Big(Z_1,Z_2,Z_3,Q_1,Q_2,\lambda\Big)$ is continuous on 
$\SH_2\times\SH_2\times\SH_2\times{\rm Sym}(2,\RR)\times {\rm Sym}(2,\RR)\times\overline R_\epsilon$
and therefore bounded on a compact subset. This yields the following estimate for the second term on the right of \rf{cutoffest}, again valid for all $\lambda\in R_\epsilon$.
$$
{{1}\over{3}}\EE\left[\chi\Big(\|k\widehat Q_1\| \le \epsilon_1,\|k\widehat Q_2\| \le \epsilon_1, (Z_1,Z_2,Z_3)\in K\Big)\Sigma\right]
\le C(\epsilon,\epsilon_1,K).
$$

The last two terms on the right of \rf{cutoffest} are handled identically, so we will focus on the third term. This is where the assumption of low disorder, i.e., that $k$ is sufficiently small, enters. We wish to exploit the fact that $\chi\left(\|k\widehat Q_1\| > \epsilon_1\right)\rarr 0$ as $k\rarr 0$, pointwise in $Q_1$. To do this we will need the following upper bound for $\Sigma$.
$$\displaylines{\quad\quad
\Sigma\Big(Z_1,Z_2,Z_3,Q_1,Q_2,\lambda\Big)
\hfill\cr\lastdisplayline{sigmaupper}{\hfill
\le
C\left(1+\|Q_1\|^{2(1+p)}+\|Q_2\|^{2(1+p)}\right)\Big(w_p(Z_1) + w_p(Z_2) + w_p(Z_3) + 1\Big)
}\quad\quad}
$$
Before proving this inequality, let us see how it can be used to complete the proof. Recall that $\widehat Q$ denotes $\Ymh_\lambda Q \Ymh_\lambda$ so that $\|\widehat Q\| \le C \|Q\|$ with $C$ uniform for $\lambda\in R_\epsilon$. Thus, using \rf{sigmaupper} and the independence of the random variables $Q_1, Q_2,Z_1, Z_2, Z_3$ we find that for bounded $k$ there exists a constant $C$ such that
$$\displaylines{\quad\quad
\EE\left[\chi\Big(\|k\widehat Q_1\| > \epsilon_1\Big)\Sigma \right]
\hfill\cr\hfill
\eqalign{
&\le C\EE_{Q_1,Q_2}\left[\chi\Big(\|k\widehat Q_1\| > \epsilon_1\Big)\left(1+\|Q_1\|^{2(1+p)}+\|Q_2\|^{2(1+p)}\right)\right]
\Big(3\EE\left[w_p(Z(\lambda))\right]+1\Big)\cr
&=\delta(k,\epsilon_1)\Big(\EE\left[w_p(Z(\lambda))\right]+1\Big)\cr
}
\quad\quad}$$
where $\delta(k,\epsilon_1)\rarr 0$ as $k\rarr 0$. Given \rf{Qhyp}, this follows from the Lebesgue dominated convergence theorem applied to $\EE_{Q_1,Q_2}\left[\chi\Big(\|k\widehat Q_1\| > \epsilon_1\Big)\left(1+\|Q_1\|^{2(1+p)}+\|Q_2\|^{2(1+p)}\right)\right]$. Combining this estimate with the previous estimates for the first and second terms on the right of \rf{cutoffest} we obtain
$$\eqalign{
\EE[w_p(Z(\lambda))] &\le (1-\delta+\delta(k,\epsilon_1))\EE[w_p(Z(\lambda))] + C\cr
&\le (1-\delta/2)\EE[w_p(Z(\lambda))] + C\cr
}$$
for $k$ sufficiently small, valid for all $\lambda\in R_\epsilon$. Since the constants here are independent of $\lambda\in R_\epsilon$, this implies the bound of \thmrf{mainest} and completes the proof, provided we can rule out $\EE[w_p(Z(\lambda))]=\infty$.

It remains to establish \rf{sigmaupper} and to prove an a priori estimate for $\EE[w_p(Z(\lambda))]$.

We begin by proving \rf{sigmaupper}. \thmrf{mainformula} and \thmrf{mainineq} imply that
$w_p\left(\Psi_\lambda\left({{Z_1+Z_2}\over{2}}\right)\right) \le \half w_p(Z_1)+\half w_p(Z_2)$.
Repeated applications of this inequality, together with \thmrf{imwt} (iv) with any choice of $\epsilon$, which we write in the less precise form $w_p(Z-Q)\le C(1+\|Q\|^{2(1+p)})(w_p(Z)+1)$, yield
$$\eqalign{
\Sigma\Big(Z_1,&Z_2,Z_3,Q_1,Q_2,\lambda\Big)
\le \sum_{\sigma}\left[ \half w_p(Z_{\sigma_1}- Q_1) + {{1}\over{4}}w_p(Z_{\sigma_2}- Q_2) +  {{1}\over{4}}w_p(Z_{\sigma_3})\right]\cr
&\le \sum_{\sigma}\left[ C(1+\|Q_1\|^{2(1+p)})(w_p(Z_{\sigma_1})+1) + C(1+\|Q_2\|^{2(1+p)})(w_p(Z_{\sigma_2})+1) + {{1}\over{4}}w_p(Z_{\sigma_3})\right]\cr
}$$
This implies \rf{sigmaupper}.

Finally we turn to the a priori bound. We need to prove $\EE[w_p(Z(\lambda))]\le C(\lambda)$, where the constant $C(\lambda)$ may blow up as $\Im \lambda$ becomes small. We will show that for any realization of the potential, 
\be{tennis}
w_p(Z(\lambda))\le C(\lambda)(1+\|Q\|^{2(1+p)}).
\ee
where $C(\lambda)$ does not depend on the potential. Then the bound follows by taking the expectation.

For this bound it is more convenient to work with the orginal forward Green function $G(\lambda)$.
By \thmrf{imwt}(i) we have $w_p(Z(\lambda))=w_p(Z(\lambda),iI)=w_p(G(\lambda),G_\lambda)$. For any realization of the potential, the recursion relation can be written $G(\lambda)=-(G_1+G_2+\lambda-\L_G-Q)^{-1}$, where we are writing $G_i$ for $G_i(\lambda)$. Thus
$$
\|G(\lambda)\| \le \sup_{Z\in S\HH_2}\|(Z+i\Im\lambda)^{-1}\| \le C/\Im\lambda
$$
(see \thmrf{isthisobvious} in the Appendix for the second inequality). The same estimate holds for $\|G_1\|$ and $\|G_2\|$. Now let $Y_1=\Im(G_1+G_2+\lambda-\L_G-Q)$ and $Y_2 = \Im(2G_\lambda+\lambda-\L_G)$. Notice that for $i=1,2$, $Y_i\ge\Im\lambda$ and so, since $Y_i$ is real symmetric,$Y_i^{-1}\le 1/\Im\lambda$. Now we use the invariance of $w_p$ in \thmrf{imwt}(i), and the fixed point property of $G_\lambda$ to write
$$\eqalign{
w_p(G(\lambda),G_\lambda) &= w_p(-(G_1+G_2+\lambda-\L_G-Q)^{-1},-(2G_\lambda+\lambda-\L_G)^{-1})\cr
&=w_p(G_1+G_2+\lambda-\L_G-Q,2G_\lambda+\lambda-\L_G)\cr
&=\|Y_2^{-1/2}(G_1^*+G_2^*-Q-2G_\lambda^*)Y_1^{-1}(G_1+G_2-Q-2G_\lambda)Y_2^{-1/2}\|_{1+p}^{1+p}\cr
&\le \Big( \Im\lambda^{-1}(\|G_1\|_{1+p}+\|G_2\|_{1+p}+\|Q\|_{1+p}+2\|G_\lambda\|_{1+p})\Big)^{2(1+p)}\cr
&\le \Big( \Im\lambda^{-1}(C/\Im\lambda+\|Q\|_{1+p}+2\|G_\lambda\|_{1+p})\Big)^{2(1+p)}\cr
}$$
Since $\|G_\lambda\|_{1+p}$ is a $\lambda$ dependent constant, independent of the potential, and all norms are equivalent for $2\times 2$ matrices, this inequality implies \rf{tennis}
\endproofof

Our next task is to reduce \thmrf{mu3est} to a statement about $\mu_{2,p}^*$.

The standard compactification $\overline\SH_2$ of $\SH_2$ is obtained by using the ball model.
This is the set of all symmetric $2\times 2$ complex matrices $W$ with $\|W\| < 1$. Here the norm is the operator norm, $W$ being regarded as an operator on a two dimensional $\ell^2$ space. The upper half space model and the ball model are related by the map $Z\mapsto (Z-iI)(Z+iI)^{-1}=(Z+iI)^{-1}(Z-iI)$ and its inverse. The ball model can be compactified in a natural way, by taking its closure in the Euclidean topology. The boundary of this closure, which we identify with the boundary at infinity, $\PA_\infty \SH_2$, of $\SH_2$, contains all symmetric $2\times 2$ complex matrices $W$ with $\|W\| = 1$  Thus, ${\overline\SH_2} = \SH_2 \cup \PA_\infty \SH_2$. For more information, see [F]. We now extend $\mu_3$ to the compactification ${\overline\SH_2}\times{\overline\SH_2}\times{\overline\SH_2}\times{\rm Sym}(2,\RR)\times {\rm Sym}(2,\RR)\times\overline R_\epsilon$ by defining its value at a boundary point as the supremum of all values along all sequences converging to the boundary point in the topology of the compactification. Since the resulting function is upper semicontinuous, \thmrf{mu3est} follows if we show that the value of $\mu_3$ on any point of the boundary 
${\overline\SH_2}\times{\overline\SH_2}\times{\overline\SH_2}\times\{0\}\times \{0\}\times J$ is $<1$. Recall that $J$ is the real interval at the base of $R_\epsilon$. 

First, let us show that $\mu_3 \le 1$ on the boundary. Let $(Z_1,Z_2,Z_3)\in\PA_\infty(\SH_2\times\SH_2\times\SH_2)$ (this means that at least one $Z_i$ is in
$\PA_\infty \SH_2$) and $\lambda\in J\subset\RR$. To estimate the value of $\mu_3$ at the boundary point $(Z_1,Z_2,Z_3,0,0,\lambda)$ let $(Z_{1,n},Z_{2,n},Z_{3,n},Q_{1,n},Q_{2,n},\lambda_n)$ converge to this point in the topology of the compactification. We must bound $\mu_3$ along this sequence.

A calculation together with the inequality \rf{mucomp} shows that
$$
\displaylines{\quad
\mu_3(Z_{1},Z_{2},Z_{3},Q_{1},Q_{2},\lambda)
=
\sum_{\sigma}\mu_{2,p}^*\left(Z_{\sigma_1}-2Q_1,\Psi_\lambda\left(\half Z_{\sigma_2}+\half Z_{\sigma_3} - Q_2\right)\right)
\hfill\cr\hfill\lastdisplayline{mu3mu2}{
\times\left(
{{\displaystyle{{{1}\over{2}}} w_p(Z_{\sigma_1}-2Q_1) + \displaystyle{{{1}\over{4}}}\mu_{2,p}^*(Z_{\sigma_2}-Q_2,Z_{\sigma_3}-Q_2)
(w_p(Z_{\sigma_2}-Q_2) + w_p(Z_{\sigma_3}-Q_2))}
\over
{w_p(Z_1)+ w_p(Z_2)+ w_p(Z_3)}}
\right).\quad\quad
}}$$

By \thmrf{mainineq} we know $\mu_{2,p}^*\le 1$ so when evaluated at $(Z_{1,n},Z_{2,n},Z_{3,n},Q_{1,n},Q_{2,n},\lambda_n)$,
$$
{
\mu_3
\le
\sum_{\sigma}
\left(
{{\displaystyle{{{1}\over{2}}} w_p(Z_{\sigma_1,n}-2Q_{1,n}) + \displaystyle{{{1}\over{4}}}
(w_p(Z_{\sigma_2,n}-Q_{2,n}) + w_p(Z_{\sigma_3,n}-Q_{2,n}))}
\over
{w_p(Z_{1,n})+ w_p(Z_{2,n})+ w_p(Z_{3,n})}}
\right).
}
$$
Thus by \thmrf{imwt} (iv), since $Q_{1,n},Q_{2,n}$ tend to zero, the limit is $\le 1$. 

Since the symplectic action $Z\mapsto Z+Q$ for $Q\in{\rm Sym}(2,\RR)$ extends continuously to the boundary at infinity, the sequence $Z_n + Q_n$ will converge to $Z$ in the compactification if $Z_n\rarr Z$ and $Q_n\rarr 0$. Thus \rf{mu3mu2} implies that if $\mu_3\rarr 1$ along a sequence converging to $(Z_1,Z_2,Z_3,0,0,\lambda)$ in the compactification, then there are sequences
$Z_{1,n}\rarr Z_1$, $Z_{2,n}\rarr Z_2$, $Z_{3,n}\rarr Z_3$ and $\lambda_n\rarr\lambda$ such that
\be{mu2is1.1}
\mu_{2,p}^*(Z_{1,n},Z_{2,n})\rarr 1, \quad \mu_{2,p}^*(Z_{1,n},Z_{3,n})\rarr 1, \quad \mu_{2,p}^*(Z_{2,n},Z_{3,n})\rarr 1,
\ee
and
\be{mu2is1.2}\eqalign{
\mu_{2,p}^*\left(Z_{1,n},\Psi_{\lambda_n}\left({{Z_{2,n}+Z_{3,n}}\over{2}}\right)\right)&\rarr 1, \cr 
\mu_{2,p}^*\left(Z_{2,n},\Psi_{\lambda_n}\left({{Z_{3,n}+Z_{1,n}}\over{2}}\right)\right)&\rarr 1, \cr 
\mu_{2,p}^*\left(Z_{3,n},\Psi_{\lambda_n}\left({{Z_{1,n}+Z_{2,n}}\over{2}}\right)\right)&\rarr 1. \cr 
}\ee
The sequences in each limit may be different.

The way one might hope to use these equations is to show that if $\mu_{2,p}^*(Z_{1,n},Z_{2,n})\rarr 1$ then the limits $Z_1$ and $Z_2$ are equal, that is
$Z_1=Z_2=Z$, and that $(Z_{1,n}+Z_{2,n})/2 \rarr Z$ too. The second statement is not automatic because addition does not extend continuously to the compactification. This would be a plausible extension of \thmrf{mainineq}, and can be shown to hold for a tree. Then \rf{mu2is1.1} and \rf{mu2is1.2} would imply that there is a $Z$ on the boundary at infinity with $\Psi_\lambda(Z)=Z$. This contradiction would prove the desired inequality and hence \thmrf{mu3est}.

This approach fails for the product graph we are considering. However the following two propositions can be used in an analogous way. The next proposition says that even though it is possible that $\mu_{2,p}^*(Z_{1,n},Z_{2,n})\rarr 1$ without $Z_1=Z_2$, the limit condition does imply that both $Z_1$ and $Z_2$ belong to the same set, an image of $\overline\HH$ imbedded in $\SH_2$ described by $(ii)$ or $(iii)$ below.

\beginpropositionlabel{notquiteequal} 

Let $(Z_{1,n},Z_{2,n})$ be a sequence converging to a point in ${\overline\SH_2}\times {\overline\SH_2}$ with $\mu_{2,p}^*(Z_{1,n},Z_{2,n})\rarr 1$. Then either

(i) $Z_{1,n}$, $Z_{2,n}$ and the average $Z_{a,n} = (Z_{1,n}+Z_{2,n})/2$ (possibly for a subsequence) all converge to the same point in ${\overline\SH_2}$. In other words, the corresponding points $W_{1,n}$, $W_{2,n}$ and $W_{a,n}$ in the ball model converge to the same point in the Euclidean topology.

(ii) There exists a real orthogonal matrix $V$ such that  $W_{i,n}\rarr V\twovec{1&0}{0&\alpha_i}V^t$ for $i=1,2,a$ (possibly for a subsequence). Here $|\alpha_i|\le 1$ and the limit $W_{i}$ lies on the boundary of the ball model.

(iii) There exists a real orthogonal matrix $V$ and $r,p \in \RR$ such that $Z_{i,n}\rarr V\twovec{z_i&r}{r&p}V^t$ for $i=1,2,a$ (possibly for a subsequence). Here $z_i\in \overline{\HH}$ and the limit $Z_{i}$ lies on the boundary of the upper half space model.
\endpropositionlabel

The next proposition says that the sets described above do not intersect their images under $\Psi_\lambda$. 

\beginpropositionlabel{nofixedset}

(i) If $Z$ lies on the boundary of $\SH_2$ in the upper half space model, then $\Psi_\lambda(Z) \ne Z$ for every $\lambda\in J$.

(ii) Suppose $V$ is a real orthogonal matrix and $V\twovec{1&0}{0&\alpha}V^t$ and $V\twovec{1&0}{0&\beta}V^t$ with $|\alpha|\le 1$, $|\beta|\le 1$ are two points in the boundary of the ball model. Then for every $\lambda\in J$
$$
\tilde\Psi_\lambda(V\twovec{1&0}{0&\alpha}V^t) \ne V\twovec{1&0}{0&\beta}V^t.
$$
Here $\tilde\Psi_\lambda$ denotes the action of $\Psi_\lambda$ conjugated to act on the ball model.

(iii) Suppose $V$ is a real orthogonal matrix and $V\twovec{z&r}{r&p}V^t$ and $V\twovec{z'&r}{r&p}V^t$ with $z,z'\in\overline{\HH}$ are two points on the boundary in the upper half space model. Then for every $\lambda\in J$
$$
\Psi_\lambda(V\twovec{z&r}{r&p}V^t) \ne V\twovec{z'&r}{r&p}V^t.
$$
\endproposition

We now show how \thmrf{notquiteequal} and \thmrf{nofixedset} imply \thmrf{mu3est} and thus our main result.

\beginproofof{\thmrf{mu3est}}
Suppose $\mu_3\rarr 1$ along a sequence $(Z_{1,n},Z_{2,n},Z_{3,n},Q_{1,n},Q_{2,n},\lambda_n)$ converging to  $(Z_1,Z_2,Z_3,0,0,\lambda)$ in the compactification. Then, there are sequences so that \rf{mu2is1.1} and \rf{mu2is1.2} hold. Then, by \thmrf{notquiteequal} there are three possibilities. (i): $Z_{i,n}$ and $(Z_{i,n}+Z_{j,n})/2$ (possibly for a subsequence) all converge to the same point $Z$ and thus $\Psi_\lambda(Z)=Z$. This is not possible since the only fixed point of $\Psi_\lambda$ in $\overline\SH_2$ is $iI$. (We leave the proof of the required continuity in $\lambda$ to the reader.) The second possibility is (ii): $Z_{i,n}$ and $(Z_{i,n}+Z_{j,n})/2$ (possibly for a subsequence) when viewed in the ball model all converge to matrices of the form $V\twovec{1&0}{0&\alpha}V^t$ for the same real rotation matrix $V$ but possibly different values of $\alpha$ with $|\alpha|\le 1$. Then \rf{mu2is1.2} implies that there exist $\alpha$ and $\beta$ with $|\alpha|\le 1$, $|\beta|\le 1$ such that $\tilde\Psi_\lambda\cdot(V\twovec{1&0}{0&\alpha}V^t) = V\twovec{1&0}{0&\beta}V^t$. This is impossible by \thmrf{nofixedset} (ii). Otherwise (iii): $Z_{i,n}$ and $(Z_{i,n}+Z_{j,n})/2$ (possibly for a subsequence) all converge to matrices of the form $V\twovec{z&r}{r&p}V^t$ for the same real rotation matrix $V$ and the same values of $r,p\in \RR$ but possibly different values of $z \in \overline\HH$. Then \rf{mu2is1.2} implies that there exist $z,z'\in\overline \HH$ such that $\Psi_\lambda\cdot(V\twovec{z&r}{r&p}V^t)=V\twovec{z'&r}{r&p}V^t$. This is impossible by \thmrf{nofixedset} (iii). Since all cases lead to a contradiction, we conclude that $\mu_3\rarr 1$ is not possible. Therefore \thmrf{mu3est} holds.
\endproofof

\endsection
\vfill\eject


==> refs.tex <==
\vfill\eject
\hd{Acknowledgements}
It is pleasure to acknowledge conversations with Jonathan Breuer who suggested that we consider this model, and the Banff International Research Station, where these conversations took place.

\hd{References}
\parindent = 0pt
\tolerance = 1000
\baselineskip = 15pt

[ASW] M.~Aizenman, R.~Sims and S.~Warzel, {\it Stability of the Absolutely 
Continuous Spectrum of Random Schr\"odinger Operators on Tree Graphs,}
Prob.~Theor.~Rel.~Fields, {\bf 136}, No.~3, 363--394, 2006, {\tt arXiv:math-ph/0502006v3}.
\medskip

[F] P.~J.~Frietas, {\it On the action of the symplectic group on the Siegel upper half plane}, Ph.D.\ Thesis, University of Illinois at Chicago, 1999 {\tt http://ptmat.fc.ul.pt/$\sim$pedro/thesis.pdf}
\medskip

[FHS] R.~Froese, D.~Hasler and W.~Spitzer, {\it Absolutely Continuous Spectrum for the Anderson Model on a Tree: A Geometric Proof of Klein's Theorem}, Comm.~Math.~Phys., {\bf 269}, No.~1, 239--257, 2007, {\tt mp-arc:05-388}.
\medskip

[FHS2] R.~Froese, D.~Hasler and W.~Spitzer,  {\it Absolutely continuous spectrum for a random potential on a tree with strong transverse correlations and large weighted loops}, Rev.~Math.~Phys., Vol.~21 no.~6, 709--733, 2009, {\tt arXiv:0809.4197v1 [math-ph]}
\medskip

[FHS3] R.~Froese, D.~Hasler and W.~Spitzer,  {\it On the AC Spectrum of One-dimensional Random Schr\"odinger Operators with Matrix-valued Potentials}, Mathematical Physics, Analysis and Geometry, 	Vol.~13, No.~3, 219--233, 2010,	{\tt arXiv:0912.0294v1 [math-ph]}
\medskip

[FHS4] R.~Froese, D.~Hasler and W.~Spitzer,  {\it A geometric approach to absolutely continuous spectrum for discrete Schr\"odinger operators}, to appear in the proceedings of the Alp workshop ``Spectral and probabilistic properties of random walks on random graphs'', Graz - St.~Kathrein, July 2009, {\tt arXiv:1004.4843v1 [math-ph]}
\medskip

[H] F.~Halasan, {\it Absolutely Continuous Spectrum for the Anderson Model on Some Tree-like Graphs,} {\tt arXiv:0810.2516v3 [math-ph]}, see also U.B.C.\ thesis {\it Absolutely continuous spectrum for the Anderson model on trees}, (2009) available at {\tt https://circle.ubc.ca/handle/2429/18857}.
\medskip

[K] A.~Klein, {\it Extended States in the Anderson Model on the Bethe
Lattice}, Advances in Math., {\bf 133}, 163--184, 1998, {\tt mp-arc:94-236}.
\medskip

[KLW] M,~Keller, D,~Lenz, S.~Warzel, private communication, the deterministic case is treated in {\it On the spectral theory of trees with finite forward cone type,} {\tt arXiv:1001.3600v1 [math.SP]}
\medskip


==> rixmax.tex <==
\input amssym.def
%\def\Bbb{\bf} %if \Bbb not available
 
%fonts

\font\bold=cmssbx10
\font\smallfont = pplr at 8.5pt
\font\smallit = pplri at 8.5pt
\font\normalfont = pplr at 9.5pt
\font\it = pplri at 9.5pt
\font\marginfont=cmr7

\def\pplfonts{
	\font\tenrm=pplr at 9.5pt
	\font\tensl=pplro at 9.5pt
	\font\eightit=pplri at 8.5 pt
	\tenrm
}


% shorthand
 
\def\larr{\leftarrow}
\def\rarr{\rightarrow}
\def\uarr{\uparrow}
\def\darr{\downarrow}
\def\PA{\partial}
\def\ti{\tilde}
\def\<{\langle}
\def\>{\rangle}
\def\cents{\hbox{\rm\rlap/c}}

% single letters

\def\HI{{\cal H}}
\def\HH{{\Bbb H}}
\def\RR{{\Bbb R}}
\def\CC{{\Bbb C}}
\def\ZZ{{\Bbb Z}}
\def\NN{{\Bbb N}}
\def\MM{{\cal M}}
\def\QQ{{\Bbb Q}}
\def\DD{{\cal D}}
\def\FF{{\cal F}}
\def\BB{{\cal B}}
\def\GG{{\cal G}}
\def\SS{{\bf S}}
\def\TT{{\bf T}}
\def\EE{{\cal E}}
\def\UU{{\cal U}}
\def\II{{\cal I}}
\def\OO{{\cal O}}
\def\Fb{{\bf F}}
\def\ib{{\bf i}}
\def\jb{{\bf j}}
\def\kb{{\bf k}}
\def\rb{{\bf r}}
\def\vb{{\bf v}}
\def\hb{{\bf h}}
% misc math stuff

\def\slim{\mathop{\hbox{\rm s-lim}}}
\def\Ker{\mathop{\rm Ker}}
\def\Ran{\mathop{\rm Ran}}
\def\ad{\mathop{\rm ad}}
\def\Re{\mathop{\rm Re}}
\def\Im{\mathop{\rm Im}}
\def\Log{\mathop{\rm Log}}
\def\Arg{\mathop{\rm Arg}}
\def\tr{\mathop{\rm tr}}
\def\curl{\mathop{\bold curl}}
\def\div{\mathop{\bold div}}
\def\ess{\hbox{\it ess}}
\def\d{\hbox{\it d}}
\def\c{\hbox{\it c}}
\def\pp{\hbox{\it pp}}
\def\jap#1{\left\langle #1 \right\rangle}
\def\sph{S^{n\kern -.2ex -\kern -.2ex 1}}
\def\half{$\scriptstyle{{1}\over{2}}$}
\def\third{$\scriptstyle{{1}\over{3}}$}
\def\quarter{$\scriptstyle{{1}\over{4}}$}
\def\DT{{{\partial}\over{\partial t}}}
\def\L{\Delta}
\def\norm#1{\|#1\|}
\def\dint{\int\hskip -5pt \int}
\def\trint{\int\hskip -5pt \int\hskip -5pt \int}
\def\amatfour#1#2#3#4#5#6#7#8{
\left[\matrix{
#1\cr
#3\cr
#5\cr
#7\cr
}\right.\left|\matrix{
#2\cr#4\cr#6\cr#8\cr
}\right]
}

\def\vec4#1#2#3#4{
\left[\matrix{
#1\cr
#2\cr
#3\cr
#4\cr
}\right]
}

\def\amatthree#1#2#3#4#5#6{
\left[\matrix{
#1\cr
#3\cr
#5\cr
}\right.\left|\matrix{
#2\cr#4\cr#6\cr
}\right]
}

\def\vec3#1#2#3{
\left[\matrix{
#1\cr
#2\cr
#3\cr
}\right]
}
 
\def\amatwo#1#2#3#4{
\left[\matrix{
#1\cr
#3\cr
}\right.\left|\matrix{
#2\cr#4\cr
}\right]
}
\def\vec2#1#2{
\left[\matrix{
#1\cr
#2\cr
}\right]
}
 
\def\threevec#1#2#3{
\left[\matrix{
#1\cr
#2\cr
#3\cr
}\right]
}

\def\twovec#1#2{
\left[\matrix{
#1\cr
#2\cr
}\right]
}

\def\tr{{\rm tr}}
\def\div{\hbox{\bold div}}
\def\curl{\hbox{\bold curl}}
% misc


%
% 	the stuff after \ifdraftmode only appears if \draftmode has previously 
%	appeared
%
\def\draftmode{\let\dfmd 1}
\def\ifdraftmode#1{\ifx\dfmd 1{#1}\fi}

\def\today{\ifcase\month\or January\or February \or March \or April\or May\or June\or July\or August\or September\or October \or November \or December\fi
\space\number\day, \number\year}

\def\nnarrower{\advance\leftskip by 30pt\advance\rightskip by 30pt}

\def\wwider{\advance\leftskip by -30pt\advance\rightskip by -30pt}

\def\quote#1{{\smallskip\nnarrower\noindent{\it#1}\smallskip}}

\def\hd#1{
\par\penalty-5000
\bigskip\bigskip{\noindent\bold #1}\par\vrule height\bigskipamount width 0pt\penalty10000
}

\def\enum#1{\par\noindent\quad\rlap{#1}\hskip 20pt}

\def\Box{\vbox{\hrule
              \hbox{\vrule height7pt\kern7pt\vrule height7pt}
              \hrule
              }
        }

\def\Picbox{\centerline{
		\vbox{\hrule
                \hbox{\vrule height2.5in\kern5in\vrule height2.5in}
                \hrule
                }
	    }
        }

% 
%	a box of specified height, width and thickness
%

\def\boxhwt#1#2#3{\vbox{\hrule width#2 height#3
                	\hbox{\vrule height#1 width#3 \kern#2\kern-#3\kern-#3 \vrule height#1 width#3}
                	\hrule width#2 height#3
                	      }
        	}
%
%
%	mcomment puts a comment in the margins
%
%
%
%
\def\strutdepth{\dp\strutbox}
%
\newdimen\pagewidth
\newdimen\marginsize

\def\margininsert#1{\strut\vadjust{\kern-\strutdepth
\vtop to \strutdepth{\baselineskip\strutdepth\vss\llap{\marginfont #1}\null}}}
%
\def\marginbox#1{{
\pagewidth=8.5 true in
%	set \marginsize to 1in + \hoffset - .26 true in
	\marginsize=1 true in
	\advance \marginsize by \hoffset
	\advance \marginsize by -.26 true in
\parindent=0pt\raggedright\hsize = \marginsize\vbox{#1}\kern 3pt}}
%
%
\def\mcomment#1{\margininsert{\marginbox{#1}}}

%
%       the following macros read in the files \jobname.eqr 
%       and \jobname .thm which 
%       contain the names of equations and how they are nested 
%       within sections in a format like 
%       \\{name1}\bgnscn\\{name2}\bgnscn\\{name3}\ndscn\ndscn
%       In this example \eqlabelname1 will expand to 1
%                       \eqlabelname2 will expand to 1.1
%                       \eqlabelname3 will expand to 1.1.1
%       This is the maximum nesting supported
%       In the theorem list each \\{name} is preceded by \typetheorem,
%       \typelemma or \typeproposition to indicate what it is
%



\def\bgnsctn{
        \advance\secnest by1
        \cntnumber=0
        \ifnum\secnest=1 
                \advance\seclevelone by1 
                \edef\prenum{\number\seclevelone .}
        \fi
        \ifnum\secnest=2 
                \advance\secleveltwo by1
                \edef\prenum{\number\seclevelone .\number\secleveltwo .}
        \fi
        }
\def\ndsctn{\advance\secnest by-1}

\def\thmtype{} %initialize
\def\typetheorem{\def\thmtype{Theorem}}
\def\typelemma{\def\thmtype{Lemma}}
\def\typeproposition{\def\thmtype{Proposition}}
\def\typecorollary{\def\thmtype{Corollary}}
\def\typehypothesis{\def\thmtype{Hypothesis}}
\def\typeconjecture{\def\thmtype{Conjecture}}
%
% first do the references - define \\ to be a macro which defines \eqlabelname 
% to be a reference number and then evaluate the input string as in Appendix D
%
\def\\#1{
        \advance\cntnumber by1
        \expandafter\xdef\csname 
        eqlabel#1\endcsname{\prenum\number\cntnumber}
        }
\newcount\seclevelone \seclevelone=0
\newcount\secleveltwo \secleveltwo=0
\newcount\cntnumber \cntnumber=0
\newcount\secnest \secnest=0
\def\prenum{}
\newread\eqrinfile 
\openin\eqrinfile=\jobname .eqr 
\ifeof\eqrinfile
  \def\eqrinput{\relax}
\else\loop
  \read\eqrinfile to\eqrinput
  \eqrinput
  \ifeof\eqrinfile\let\endfile 1\else\let\endfile 0\fi
  \ifx\endfile 0 \repeat
\fi
\closein\eqrinfile

%
% now the same thing for theorems
%
\def\\#1{
        \advance\cntnumber by1
        \expandafter\xdef\csname 
        thmlabel#1\endcsname{\prenum\number\cntnumber}
        \expandafter\xdef\csname 
        typethmlabel#1\endcsname{\thmtype\ \prenum\number\cntnumber}
        }
\seclevelone=0
\secleveltwo=0
\cntnumber=0
\secnest=0
\def\prenum{}
\newread\thminfile 
\openin\thminfile=\jobname .thm
\ifeof\thminfile
  \def\thminput{\relax}
\else\loop
  \read\thminfile to\thminput
  \thminput
  \ifeof\thminfile\let\endfile 1\else\let\endfile 0\fi
  \ifx\endfile 0 \repeat
\fi
\closein\thminfile


        
%
% theorems etc
% These are numbered by section
%

\def\begintheoremlabel#1{
       	\toksdef\ta=0
	\ta={\typetheorem\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Theorem \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endtheoremlabel{\par\medbreak\endgroup}

\def\begintheorem{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\begintheoremlabel\temp
}
\def\endtheorem{\endtheoremlabel}

\def\beginlemmalabel#1{
        \toksdef\ta=0
	\ta={\typelemma\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Lemma \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endlemmalabel{\par\medbreak\endgroup}

\def\beginlemma{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\beginlemmalabel\temp
}
\def\endlemma{\endlemmalabel}



\def\beginpropositionlabel#1{
        \toksdef\ta=0
	\ta={\typeproposition\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Proposition \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endpropositionlabel{\par\medbreak\endgroup}

\def\beginproposition{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\beginpropositionlabel\temp
}
\def\endproposition{\endpropositionlabel}

\def\begincorollarylabel#1{
        \toksdef\ta=0
	\ta={\typecorollary\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Corollary \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endcorollarylabel{\par\medbreak\endgroup}

\def\begincorollary{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\begincorollarylabel\temp
}
\def\endcorollary{\endcorollarylabel}

\def\beginhypothesislabel#1{
        \toksdef\ta=0
	\ta={\typehypothesis\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Hypothesis \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endhypothesislabel{\par\medbreak\endgroup}

\def\beginhypothesis{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\beginhypothesislabel\temp
}
\def\endhypothesis{\endhypothesislabel}

\def\beginconjecturelabel#1{
       	\toksdef\ta=0
	\ta={\typeconjecture\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Conjecture \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endconjecturelabel{\par\medbreak\endgroup}

\def\beginconjecture{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\beginconjecturelabel\temp
}
\def\endconjecture{\endconjecturelabel}





\def\beginproof{\medbreak\par\noindent{\it Proof:\/\ }}
\def\endproof{\thinspace\Box\par\medbreak}

\def\beginproofof#1{\medbreak\par\noindent{\it Proof of #1:\/\ }}
\def\endproofof{\thinspace\Box\par\medbreak}



\def\begindefn{\medbreak\par\noindent{\it Definition:\/\ }}
\def\enddefn{\par\medbreak}

\def\beginexample{\medbreak\par\noindent{\it Example:\/\ }}
\def\endexample{\par\medbreak}

\def\beginexampleset{\beginproblemset}
\def\endexampleset{\endproblemset}


\def\beginremark{\medbreak\par\noindent{\it Remark:\/\ }}
\def\endremark{\par\medbreak}

\def\beginremarkno#1{\medbreak\par\noindent{\it Remark #1:\/\ }}
\def\endremarkno{\par\medbreak}



%-------------------------------------------------------
%	no longer needed
%
%       \appendtxt appends the text in #2 to the token list 
%       contained in the token variable #1
%
\def\appendtxt#1#2{ 
        \toksdef\ta=0
        \ta=\expandafter{\the#1#2}
        \global#1=\expandafter{\the\ta}
        }
%----------------------------------------------------------

%
%
%	open files for writing
%
%
\newwrite\eqroutfile 
\immediate\openout\eqroutfile=\jobname .eqr 
\newwrite\thmoutfile 
\immediate\openout\thmoutfile=\jobname .thm


%
%       \be{name} and \ee begin and end a numbered displayed equation 
%       the tokens in the name are added to the token list in \eqrtoks
%       if \eqlabelname has been defined uses this as a number
%       \lastdisplayline{name}{...} gives a referenced number  to the last 
%       line in a displaylines series
%
\def\be#1{
        \def\temp{#1}
	\toksdef\ta=0
	\ta={\\{#1}}
        \immediate\write\eqroutfile{\the\ta}$$
	}
\def\ee{
        \eqno{(\csname eqlabel\temp\endcsname)
	\ifdraftmode{\rlap{\ {\marginfont\temp}}}}$$
        }
\def\lastdisplayline#1#2{
        \hfill#2\hfill{\rm\llap{(\csname eqlabel#1\endcsname)}
	\ifdraftmode{\rlap{\ {\marginfont#1}}}}\cr
        \toksdef\ta=0
	\ta={\\{#1}}
        \immediate\write\eqroutfile{\the\ta}
        }

%
%       \beginsection begins a new section
%       writes \bgnsctn to token list in \eqrtoks
%       \endsection ends a section
%       writes \ndsctn to token list in \eqrtoks
%
\def\beginsection{
        \advance\secnumber by1
        \probctr=0
	\toksdef\ta=0
	\ta={\bgnsctn}
        \immediate\write\eqroutfile{\the\ta}
        \immediate\write\thmoutfile{\the\ta}
        }
\def\endsection{
        \toksdef\ta=0
	\ta={\ndsctn}
        \immediate\write\eqroutfile{\the\ta}
        \immediate\write\thmoutfile{\the\ta}
        }

%
%       \rf{name} inserts (<number>) where <number> is the equation number
%       referred to by "name"
%
\def\rf#1{(\csname eqlabel#1\endcsname )}

%
%       \thmrf is the analogous thing for theorems
%
%\def\thmrf#1{\hbox{\csname typethmlabel#1\endcsname}}
\def\thmrf#1{\csname typethmlabel#1\endcsname}







\def\chead#1{\medbreak\centerline{#1}\medskip}

\def\bea#1{$$\eqalign\begingroup}
\def\eea{\endgroup $$}
\def\beann{$$\eqalign\begingroup}
\def\eeann{\endgroup $$}


%
%       some lecture note macros
%
\def\beginlecture{
        \beginsection 
        \probctr=0
        \par\noindent{\bf Lecture \number\secnumber}
        \medskip
}
\def\endlecture{\endsection\vfill\eject}
%
%
%
\def\beginlecturetitle#1{
        \beginsection 
        \probctr=0
        \par\noindent{\bf Lecture \number\secnumber : #1}
        \medskip
}
\def\endlecturetitle{\endsection\vfill\eject}
%
%
%
\def\readsec#1{\medskip{\sl Reading:} Section #1}
\def\readsecs#1{\medskip{\sl Reading:} Sections #1}
\def\hmk#1#2{\medskip{\sl Problems (due #1): }#2}
%
%       sec macro
%
\def\beginsec#1{
	\bigskip
        \beginsection 
        \par\noindent\centerline{\bf \number\secnumber . #1}
        \medskip
}
\def\endsec{\endsection\par}

\def\beginproblem{
        \advance\probctr by1
        \medbreak\par\noindent
        {\it Problem \number\secnumber .\number\probctr:\/}
}
\def\endproblem{\par\medbreak}

\def\beginquestion{
        \advance\probctr by1
        \medbreak\par\noindent
        {\it Question \number\secnumber .\number\probctr:\/}
}
\def\endquestion{\par\medbreak}

\def\ans{{\medskip\bold Answer: }}

\def\beginsolution{
        \medbreak\par\noindent
        {\it Solution \number\secnumber .\number\probctr:\/}
}
\def\endsolution{\par\medbreak}

\def\beginproblemset{\bigskip\hrule\bigskip\advance\leftskip by 30pt
\advance\rightskip by 30pt\smallfont}
\def\endproblemset{\bigskip\hrule\bigskip\advance\leftskip by -30pt
\advance\rightskip by -30pt\normalfont}
\def\bsp{\beginproblemset\beginproblem}
\def\esp{\endproblem\endproblemset}


%
%	some research note macros
%

\def\beginnote#1{
	%\magnification 1100
	\hsize = 5.9 true in
	\hoffset = 0.45 true in
	\baselineskip = 18pt
        \beginsection 
        \probctr=0
        \par\noindent\centerline{\bf #1}
	\centerline{filename: {\tt\jobname .tex}}
	\centerline{\today}
        \medskip
}
\def\endnote{\endsection\vskip 20pt}


\def\notefontsize{
	\hsize = 5.9 true in
	\hoffset = 0.45 true in
	\baselineskip = 18pt}

%
%       These go at the beginning  of input
%
\global\newtoks\eqrtoks
\global\newtoks\thmtoks
\global\newcount\secnumber
\global\newcount\nonamectr
\global\newcount\probctr



\def\rixend{\closeout\eqroutfile \closeout\thmoutfile \vfill\eject\end}

\message{*** reference macros need to run twice to get references right ***}


==> stackedtree.tex <==
\input rixmax
\input epsf
\font\text=pplr at 10pt
\font\it=pplri at 10pt
\font\bold=phvb at 10pt
%\draftmode
%\magnification 1100
        \hsize = 5.9 true in
        \hoffset = 0.45 true in
        \baselineskip = 18pt

\def\mcomment#1{}
\footline={\hfil}
\footline={\hss\tenrm\folio\hss}
\def\half{{{1}\over{2}}}
\def\hd#1{\bigskip\bigskip{\noindent\bold #1}\par\vrule height\bigskipamount width 0pt\penalty10000}
\def\HB{\overline\HH}
\def\BB{{\Bbb B}}
\def\EE{{\Bbb E}}
\def\cd{{\rm cd}}
\def\dist{{\rm dist}}
\def\SH{{\Bbb S\Bbb H}}
\def\Yh{Y^{1/2}}
\def\Ymh{Y^{-1/2}}
\def\Ran{\mathop{\rm Ran}}
\def\hdd#1{\bigskip\bigskip\noindent{\sl #1}\medskip}

\text
\centerline{\bold Absolutely continuous spectrum for the Anderson model on a product}
\vskip 10 pt
\centerline{\bold of a tree with a finite graph}
\vskip 20 pt

\centerline{Richard Froese}
\medskip
\centerline{Department of Mathematics}
%\medskip
\centerline{University of British Columbia}
%\medskip
\centerline{Vancouver, British Columbia, Canada}
\bigskip
\centerline{Florina Halasan}
\medskip
\centerline{Fakult\"at f\"ur Mathematik und Informatik}
%\medskip
\centerline{Friedrich-Schiller-Universit\"at Jena}
%\medskip
\centerline{Jena, Germany}
\bigskip
\centerline{David Hasler}
\medskip
\centerline{Department of Mathematics}
%\medskip
\centerline{Ludwig Maximilians University}
%\medskip
\centerline{Munich, Germany}

\vskip 20pt
\centerline{\today}

\input intro
\input proofs
\input appendix1
\input refs
\rixend

